FLORA: Fine-grained Low-Rank Architecture Search for Vision Transformer

Vision Transformers (ViT) have recently demonstrated success across a myriad of computer vision tasks. However, their elevated computational demands pose significant challenges for real-world deployment. While low-rank approximation stands out as a renowned method to reduce computational loads, efficiently automating the target rank selection in ViT remains a challenge. Drawing from the notable similarity and alignment between the processes of rank selection and One-Shot NAS, we introduce FLORA, an end-to-end automatic framework based on NAS. To overcome the design challenge of supernet posed by vast search space, FLORA employs a low-rank aware candidate filtering strategy. This method adeptly identifies and eliminates underperforming candidates, effectively alleviating potential undertraining and interference among subnetworks. To further enhance the quality of low-rank supernets, we design a low-rank specific training paradigm. First, we propose weight inheritance to construct supernet and enable gradient sharing among low-rank modules. Secondly, we adopt low-rank aware sampling to strategically allocate training resources, taking into account inherited information from pre-trained models. Empirical results underscore FLORA's efficacy. With our method, a more fine-grained rank configuration can be generated automatically and yield up to 33% extra FLOPs reduction compared to a simple uniform configuration. More specific, FLORA-DeiT-B/FLORA-Swin-B can save up to 55%/42% FLOPs almost without performance degradtion. Importantly, FLORA boasts both versatility and orthogonality, offering an extra 21%-26% FLOPs reduction when integrated with leading compression techniques or compact hybrid structures. Our code is publicly available at https://github.com/shadowpa0327/FLORA.

==> methods_backup.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[scale=0.47]{figs/Overview.pdf}
    \caption{Illustration of low-rank aware candidate filtering. \textbf{(a)}: Filtering is applied sequentially to each block. \textbf{(b)}: For the $i$-th transformer block, we construct a local supernet by substituting the $i$-th block with a weight-sharing superblock that encompasses the local low-rank architecture. \textbf{(c)}: Leveraging the trained supernet as a performance estimator, we filter the local rank space, considering the trade-off between performance benefits and computational costs.}
    \label{fig:/Overview}
\end{figure*}


%\section{Method}
\label{sec:method}
%To formulate the rank selection problem as supernet-based One-Shot NAS paradigm we have to design the three key components: (1). Low-rank search space ; (2) supernet construction and training; 



\section{Problem Formulation}

To introduce the low-rank approximation to the transformer, we want to substitute the linear components with their corresponding low-rank approximated linear calculation. Giver the rank setting $r$, the linear component can be approximated by two small matrices $U_r \in \mathbb{R}^{m \times r}$ and $V_r \in \mathbb{R}^{n \times r}$. If we choose a sufficient small $r < \frac{mn}{m+n}$, the number of parameters and FLOPs of each linear module are reduced from $\mathcal{O}(mn)$ to $\mathcal{O}(rm + rn)$. To harness the efficacy while maintain the competitive performance, we aim to search for a suitable rank setting $r$. 

In this work, offers an innovative approach to address rank selection by redefining it as a Neural Architecture Search (NAS) problem. This reframing is guided by a key insight: the rank settings determine the architecture of the resulting low-rank model. Furthermore, drawing from the inherent properties of SVD-based low-rank approximation, we propose a solution using the well-established branch known as One Shot NAS. 

In the weight-sharing based One-Shot NAS paradigm, the architecture search space $\mathcal{A}$ is encoded into an over-parameterized supernet $\mathcal{N}(\mathcal{A}, W)$, where $W$ stands for the weight of supernet and $W$ is shared among candidate architectures (i.e., low-rank architectures $a \in \mathcal{A}$ ). One Shot NAS paradigm comprises two main stages. First, we train the supernet by maximizing the objective function:
\begin{equation}
    \label{SPOS training}
    W_{\mathcal{A}} = \underset{W}{\text{argmin}} \mathbb{E}_{a \thicksim \Gamma(\mathcal{A})} [ \mathcal{L} (\mathcal{N}(a, W(a)) ],
\end{equation}
where $W_{\mathcal{A}}$ is the weights of the supernet, $a \in \mathcal{A}$ is a rank configuration, $W(a)$ is weights of $a$, $\mathcal{N}(a, W(a))$ denotes the corresponding subnetwork, and $\mathcal{L}$ stands for the training loss. 

Second, with the well-trained supernet, we can leverage it as a confident proxy to guide the searching algorithm such as evolutionary algorithm (EA) to search for optimal low-rank architecture that maximize the objective function (e.g., accuracy) while statisfying the target constraint (e.g, FLOPs). The objective function can be formulated as below: 
\begin{equation}
\begin{aligned}
    \label{SPOS searching}
    & a^* = \underset{a \in \mathcal{A}}{\text{argmax}}\text{ACC}_{\text{val}} (\mathcal{N} (a, W_{\mathcal{A}}(a))) \\
    &\text{s.t.} \quad \mathcal{F}_{lower} \leq \mathcal{F}(a) \leq \mathcal{F}_{upper},
\end{aligned}
\end{equation}
where $\text{ACC}_{\text{val}}$ is the accuracy on validation set, $\mathcal{F}(a)$ denotes the FLOPs of the subnetwork with the rank configuration $a$, $\mathcal{F}_{lower}$ and $\mathcal{F}_{upper}$ are the lower bound and upper bound of FLOPs constraints, respectively.


\paragraph{Challenge} Traditional One-Shot NAS methodologies often focus on a discrete search space with around 3-5 choices per block, which is deemed manageable in terms of computational demand. However, when we consider the realm of rank selection for low-rank approximation, the scenario becomes vastly more intricate, since the candidate rank choices is usually soaring beyond hundreds. 

Earlier studies focused on low-rank approximation for CNNs suggest a simplification of this astounding search space. They advocate for ranks adhering strictly to a constant multiple, often 32 or 64, aiming to strike an optimal balance between search cost and granularity \cite{DBLP:conf/aaai/Xiao0GYSXT023}. However, when these methods are applied to architectures like ViT, the sheer scale of the search space remains overwhelming. For instance, the classic DeiT-B, with its embedding dimension of 768 and a constant multiple of 64, still presents up to 12 rank choices for each linear module.

This expansive choice set introduces two primary challenges. Firstly, without a well-designed strategy to construct and train the supernet, subnetworks may risk undertraining or face weight-coupling issues \cite{DBLP:conf/iccv/Chu0X21, DBLP:journals/corr/abs-1904-00438}. This can lead to biased estimations of network performance. Secondly, once an approximate model has been identified, retraining is often essential to refine its performance – an additional computational overhead that is not desirable, especially in compression scenarios.



%\subsection{Low-Rank Aware Architecture Search}
%\subsection{Low-Rank Search Space} 



%Considering the well-knowed DeiT-S, with 12 blocks and each with 3 compression target, we can reduce the size of the search space from astounding $10^{93}$ to $10^{28}$. 



\section{Methodology}

%Our objective is twofold. 
To overcome the design challenge mentioned above, we present the poposed LORANAS, an end-to-end One-Shot NAS based solution optimized specific for rank selection problem of ViT. We offer a robust strategy to enhance the performance of low-rank supernets, including the filtering strategy to identify weak candidates to prevent from possible interferencing (Sec. \ref{sec:Local Filtering}) and alongside low-rank aware paradigm for supernet consruction and training crafted for resource efficiency and accelerated convergence based on the observation of inherent property of low-rank approximation (Sec. \ref{Sec: Supernet Boosting}). 

%In the following subsections, we first introduce design strategy of search space  (Sec. \ref{sec: search space}), follow 
%\subsection{Simplify Low-Rank Search Space}
%\label{sec: search space}
%Without loss of generality, unlike traditional settings that investigate different computational modules that could lead to varying performances, rank choices within a given range (e.g., rank choices from 24$\sim$32) are homogeneous. Thus, to mitigate the computation overhead, we make a trade-off between exploration granularity and efficiency by constrainting our exploration by exclusively considering rank settings that adhere to a constant multiple. Typically the multiple is set at 32, 64 or 96, considering the maximum rank values of each compression target to ensure sufficient coverage. 

%While this simplification strategy undeniably alleviates exploration overhead, for larger ViT models, the resulting search space remains vast. Taking the classic DeiT-B as an illustration, which has an embedding dimension of 784 and a multiple constant set to 64, we still face up to 12 rank choices for each linear module. This underscores the pressing need for advanced optimization techniques to further diminish the supernet's computational burden.

%In our effort to enhance the efficiency of Neural Architecture Search (NAS), we present LORANAS. Central to this methodology is the recognition that the search space for potential low-rank architectures is both expansive and intricate. 
%To systematically navigate this space, we adopt a bi-level strategy: initiating with a relaxation at the local component (block) level, then building upon these insights to address the global challenge comprehensively. %可能可以改的更好！

\subsection{Low-Rank Aware Candidate Filtering}
\label{sec:Local Filtering}
Supernet performance is deeply linked to the quality of its search space. 
When employing low-rank approximation, aggressive rank settings can sometimes lead to irreversible information losses. 
Conversely, architectures with overly conservative rank settings might not deliver any substantial benefits in terms of computational efficiency. The weight-sharing nature of supernets further complicates this, as tightly coupled subnetwork weights can negatively influence promising architectures, leading to interference and compromised performance.

A seemingly straightforward solution would be to discard these unsuitable configurations. However, the vastness of the low-rank search space renders such a direct approach both cumbersome and computationally taxing. To address this, we draw on a key observation: architectures that underperform at the local level (withing one transformer block) often falter in a global context (entire low-rank architecture). With this in mind, we introduce a bi-level filtering mechanism, called \textit{low-rank aware candidate filtering}, to identify architectures that strike a balance between accuracy and computational demand. 


\paragraph{Local Level Filtering} Our strategy commences at the local level, focusing on individual transformer blocks. Technically, we create a local supernet that encompasses the low-rank architecture of the current transformer block, leaving other blocks uncompressed. This local supernet is then trained on a proxy dataset—a subset of the original training data. Impressively, by using just 10\% of the original dataset, this supernet can be trained to serves as an effective estimator in roughly 10\% of the time required for comprehensive global supernet training. 

To steer our selection process, we employ the Precision Cost Ratio, defined as:
\begin{equation}
\mathcal{M}(a) = \lambda * \mathcal{P}(a) - \mathcal{F}(a)
\end{equation}
Here, $\mathcal{P}(a)$ and $\mathcal{F}(a)$ respectively denote the classification accuracy and computational overhead associated with a low-rank architecture $a$. The parameter $\lambda$ adjusts the balance between precision and cost. Utilizing this metric, we rank the low-rank architecture on a block level and retain only the top-$k$ candidates.

\paragraph{Global Level Integration} 
According to the results of local filtering, we then generated the potential global architectures based on the cartesian product. In essence, any global architecture that houses a locally discarded component is eliminated. By doing so, we effectively weeds out underperforming candidates, giving rise to a optimized search space, which is smaller and more friendly for supernet construction and training.







\begin{figure}[hpt]
    \centering
    \includegraphics[scale=0.5]{figs/LRLinear.pdf}
    \caption{Illustration of weight inheritance technique for supernet construction. All rank architecture of a specific linear modules are encompassed within a superblock. For a designated rank settings, the corresponding rank architecture will be generated by inheriting from superblock}
    \label{fig:LRLinear}
\end{figure}

\subsection{Boosting Low-Rank Supernet}
\label{Sec: Supernet Boosting}
Achieving a superior supernet performance involves multiple aspects. While refining the search space is crucial, the way subnetworks are incorporated and trained within the supernet is equally important. The successful convergence of the supernet, and its ability to prepare low-rank subnets for immediate use without additional training, depends on both the integration method and the training strategy.
%However, up to our best knowledge, there are not yet a sound strategy for low-rank supernet. 
To address these challenges, we introduce the \textit{Low-Rank Aware Training Paradigm} (LRAT). Tailored for low-rank architectures, LRAT combines two main principles: \textit{Weight Inheritance}, which ensures a suitable integration of various rank choices, and \textit{Low-Rank Aware Sampling}, a training approach that adjusts to the needs of different rank architectures.


\paragraph{Weight Inheritance} 
For each linear component with $N$ rank level choices $\mathbb{C}= \{r_1, r_2, ... , r_N\}$ and corresponding low-rank module set $\mathbb{S}= \{(U_{r_1}, V_{r_1}), (U_{r_2}, V_{r_2}) , ... , (U_{r_N},  V_{r_N})\}$, our goal is to design a suitable technique to integrate all of these candidates into a choice block. To realize this, we leverage the properties of Singular Value Decomposition (SVD). In conventional SVD, eigenvalues are sequentially ordered from the largest to the smallest on the diagonal. Thus, for a designated rank choice $k$, the most significant eigenvectors are naturally chosen to approximate the original modules. As we try out different rank options, these influential eigenvectors tend to stay consistent across various rank settings. Building on this inherent property of SVD, the convergency of low-rank modules can be faciliate via a gradient sharing strategy.

Drawing inspiration from earlier NAS practices \cite{DBLP:conf/pkdd/StamoulisDWLPLM19, DBLP:conf/iclr/YuYXYH19}, which employed shared convolutional kernels within their network structures, we adapted these strategies for our low-rank approximation, leading to the \textit{weight inheritance} method. As illustrated in Fig. \ref{fig:LRLinear}, every low-rank module is encompassed within the largest rank choice, expressed as:
\begin{equation}
\label{Eq:Weight inheritance1}
U_{r_i} = U_{r_N}[:, : r_i],
\quad V_{r_i} = V_{r_N}[:, : r_i]
\end{equation}

For a specific rank $r_i$, the values of $U_{r_i}$ and $V_{r_i}$ inherit from the top-$r_i$ columns of $U_{r_N}$ and $V_{r_N}$ respectively. During the backward pass, the gradients of $U_{r_i}$ and $V_{r_i}$ are updated back to the corresponding sub-matrices in $U_{r_N}$ and $V_{r_N}$. Within each choice block, the candidate with the largest rank is initialized using SVD, matching the size of the uncompressed model's factorized weights.

It's evident that each sub-structure is a subset of the structures with higher rank levels, culminating in the super-matrix, as shown below: 
\begin{equation}
\label{Eq:Weight inheritance2}
\begin{gathered}
    U_{r_i} \subseteq U_{r_k} ,\quad V_{r_i} \subseteq V_{r_k} \\
    \forall k \in\{i+1, i+2, ..., N\} \quad \forall r_i \in \mathbb{C}
\end{gathered}
\end{equation}
With shared weights among low-rank modules, gradient information can be efficiently utilized across groups. This mutual gradient update strategy ensures that all candidate low-rank architectures are trained concurrently, bolstering convergence during the supernet training phase.

%For a specific rank $r_i$, the values of $U_{r_i}$ and $V_{r_i}$ inherit from the top-$r_i$ columns of $U_{r_N}$ and $V_{r_N}$ respectively. During the backward pass, the gradients of $U_{r_i}$ and $V_{r_i}$ are updated back to the corresponding sub-matrices in $U_{r_N}$ and $V_{r_N}$. Within each choice block, the candidate with the largest rank is initialized using SVD, matching the size of the uncompressed model's factorized weights.
\iffalse
It is evident that each sub-structure is also the sub-matrix of the all the structure with larger rank level, including the super-matrix:
\begin{equation}
\label{Eq:Weight inheritance2}
\begin{gathered}
    U_{r_i} \subseteq U_{r_k} ,\quad V_{r_i} \subseteq V_{r_k} \\
    \forall k \in\{i+1, i+2, ..., N\} \quad \forall r_i \in \mathbb{C}
\end{gathered}
\end{equation}

Since the weights of each low-rank modules are shared, the gradient information can be leveraged among the groups. Updating the weights of smaller low-rank modules synchronously updates the larger ones and vice versa.
Under the weight inheritance strategy, all candidate low-rank architectures can be trained simultaneously, resulting in superior convergence during the supernet training.
\fi

\paragraph{Low-Rank Aware Sampling}
Contrary to prior works \cite{DBLP:conf/eccv/GuoZMHLWS20, DBLP:conf/iccv/ChenPFL21} that train the supernet from scratch, our approach initializes the supernet with weights from a pretrained uncompressed model. In this context, subnetworks are seen as low-rank approximated networks for different rank choices. This introduces a new perspective on sampling during training: it's suboptimal to sample subnetworks using a uniform distribution. Instead, our design for a new sampling distribution is guided by two key observations:
\begin{itemize}
    \item Architectural search algorithms are inherently intricate and challenging to train. Given a predetermined search space, it's computationally arduous to thoroughly train every substructure. For the entire system to achieve peak performance and consistent convergence, training resources must be judiciously allocated to different subnetworks, warranting a non-uniform distribution.
    \item Low-rank architectures, especially those of lower ranks, derive varying degrees of information from pretrained weights. Such inheritance can be perceived as the architecture having undergone preliminary training. As a result, during supernet training, it's crucial to divert more resources (like sampling probability) towards these less-informed structures, ensuring balance.
\end{itemize}
With the above insights in mind, we introduce a non-uniform path sampling strategy that favors smaller rank choices within each low-rank linear layer.
Formally, let's define the rank choice for a low-rank linear layer by a random variable $X$. 
Its Probability Mass Function (PMF) of $X$ is formulated as:
\begin{equation}
\label{Eq:NUS}
\text{$ p_X(r) = P(X=r) = \frac{\frac{1}{r}}{\sum_{r'\in \mathbb{C}}\frac{1}{r'}} ,\ \ \  \ \ r \in \mathbb{C} $}
\end{equation}
Recall that $\mathbb{C}$ denotes the rank choice set of a specific low-rank linear layer. The prior distribution of selecting a sequence of rank choice would be $\Gamma(\mathcal{A}) = P(X_1 = r_{k_1}, ..., X_i = r_{k_i} , ..., X_l = r_{k_l})$, where $X_i, r_{k_i}$ denotes the random variable of $i$-th choice block and its correlated rank choice, respectively.

%this
%well-trained supernet guides the search algorithm, such as
%an evolutionary algorithm (EA). 


%we train an over-parameterized supernet, encompassing various candidate architectures. Second, this well-trained supernet guides the search algorithm, such as an evolutionary algorithm (EA), to seek for optimal architecture that maximize the accuracy while  


%This process is efficient as architecture performance can be estimated by querying the trained supernet.







%To enhance the search performance and enable comprehensive exploration within the low-rank search space, we develop an effective framework for low-rank architecture that incorporates the following operations. Initially, we design an expansive search space to facilitate detailed exploration. We construct a memory-efficient supernet using weight inheritance techniques. Subsequently, we introduce the concept of \textit{Hieracical Rank Search}, where we first locally identify promising candidate rank settings within each encoder block, followed by a global exploration to determine the final low-rank model considering the dependency among each encoder blocks. Lastly, we adopt a low-rank-aware sampling rule when training the supernet to enable proper training resource distribution. The general overview of our framework is summarized in Fig \ref{fig:Overview}.
%The general overview of our framework is outlined in Fig 2.  


%Inspired by prior approaches, we propose to solve the low-rank decomposition design guided by a one-shot NAS scheme, which can automatically generate a more fine-grained configuration instead of handcrafting it. To formulate it into a one-shot NAS problem, we need to answer the following questions: 
%1) How to introduce low-rank as a unique and unexplored feature that is orthogonal to existing ones? 
%2) How to effectively train a supernet initialized with the pre-trained weights?

%To answer these questions, we formulate an end-to-end framework for automatic compression consisting of three stages: (I) building a supernet with weight inheritance low-rank linear layers as choice blocks (Sec \ref{Sec:Search Space}, \ref{Sec:Building}); (II) sampling subnetworks with a non-uniform sampling strategy and training them with soft label distillation (Sec \ref{Sec:Training}); and (III) searching for the optimal subnetworks with an evolutionary algorithm (Sec \ref{Sec:Searching}). Based on our framework, we successfully introduce low-rank approximation into the search space; through weight inheritance and non-uniform sampling, we further support supernet training and acquire efficient low-rank ViTs with competitive performance.
%Inspired by the fundamental of neural architecture search, we build the automatic compression framework with three stages to compress Transformer with low-rank approximation: (1) building a supernet with weight inheritance low-rank linear layers as choice blocks; and (2) sampling sub-networks with non-uniform sampling strategy and training them with soft-label distillation; and (3) searching for the optimal sub-networks through  the evolutionary algorithm.


%Based on NAS, low-rank approximation show the promising result on various types of Vision Transformers; besides, equipped with our proposed supernet training  strategy, the supernet performance is promoted an



%\subsection{Preliminary}

%\paragraph{Vision Transformer}\label{sec:Transformer} For a given input 2D image, ViT first splits it into several fixed-size patches. These patches are then flattened and linearly embedded into the sequence input, just like the sequence of tokens in NLP tasks. Position embeddings are added to the embedded input to retain positional information. Following by interleaved multi-head self-attention and multi-layer perception (MLP) modules, the critical information inside an image is aggregated into a compact feature step-by-step for final classification.

%Following the previous work from NLP to learn the global correlation between all input tokens, MHSA module first linearly projects the input patches into query ($Q$), key ($K$), and value ($V$) features, then splits them into different heads and performs self-attention in parallel. For each self-attention, it computes the weighted sum over all value features with the pair-wise attention score acquired by the inner product of the query and key features.

%\begin{equation}
%\text{$ \text{Attention}(Q_h, K_h, V_h) = \text{Softmax}(\frac{Q_h{K}_h^T}{\sqrt{d_h}}), $}
%\end{equation} where the $Q_h \in \mathbb{R}^{d\times d_h}, K_h \in \mathbb{R}^{d\times d_h}, V_h \in \mathbb{R}^{d\times d_h}$ denoted the splitted query, key, and value of head $h$, while $d$ is the embedding dimension, $d_h$ is the Q-K-V dimension. Lastly, each head's result is concatenated and linearly projected to be the final output.

%Now, let us look into the operation of the MLP module. Inside the MLP module, the input is first transformed into a hidden dimension with the first linear layer, activated with a non-linear function, usually GELU \cite{DBLP:journals/corr/HendrycksG16}, and then projected back to the original embedded dimension with the second linear layer. 
%In the following section, we will denote the first and second linear layers with FC1 and FC2, respectively.


%\paragraph{Low-Rank Approximation for Linear layer}
%\label{Low-rank approximation for Linear layer}
%Low-rank approximation is a structured pruning method that approximate a matrix $W \in \mathbb{R}^{m \times n} $ with two small matrices $ U_k \in \mathbb{R}^{m \times k} $ and $ V^T_k \in \mathbb{R}^{k \times n}$ where $k \in \mathbb{Z}^+$ is given remaining rank and $k \le min(m,n)$.
%To generate the low-rank approximated matrices, singular value decomposition (SVD) is the most well-known methodology, that we can resort to.
%Some other work further proposed the modification to reduce the information loss of SVD.
%Based on SVD, some other works further introduced  to reduce the information loss casued by the low-rank fatorization.

% Move to preliminary
%Howerve, the ways to decide is not yet well study, thus propose Trimsformer


%\paragraph{Low Rank Approximation} We can have the singular value decomposition equation here.

%\paragraph{One-shot NAS} We can briefly introduced the One-shot NAS idea here


%\paragraph{Low rank property in vision transformer.}  We can use the heatmap to state the low rank property here.



